A Survey on Automated Diagnosis of Alzheimer's Disease Using Optical Coherence Tomography and Angiography

Retinal optical coherence tomography (OCT) and optical coherence tomography angiography (OCTA) are promising tools for the (early) diagnosis of Alzheimer's disease (AD). These non-invasive imaging techniques are cost-effective and more accessible than alternative neuroimaging tools. However, interpreting and classifying multi-slice scans produced by OCT devices is time-consuming and challenging even for trained practitioners. There are surveys on machine learning and deep learning approaches concerning the automated analysis of OCT scans for various diseases such as glaucoma. However, the current literature lacks an extensive survey on the diagnosis of Alzheimer's disease or cognitive impairment using OCT or OCTA. This has motivated us to do a comprehensive survey aimed at machine/deep learning scientists or practitioners who require an introduction to the problem. The paper contains 1) an introduction to the medical background of Alzheimer's Disease and Cognitive Impairment and their diagnosis using OCT and OCTA imaging modalities, 2) a review of various technical proposals for the problem and the sub-problems from an automated analysis perspective, 3) a systematic review of the recent deep learning studies and available OCT/OCTA datasets directly aimed at the diagnosis of Alzheimer's Disease and Cognitive Impairment. For the latter, we used Publish or Perish Software to search for the relevant studies from various sources such as Scopus, PubMed, and Web of Science. We followed the PRISMA approach to screen an initial pool of 3073 references and determined ten relevant studies (N=10, out of 3073) that directly targeted AD diagnosis. We identified the lack of open OCT/OCTA datasets (about Alzheimer's disease) as the main issue that is impeding the progress in the field.

==> discussion_bkup.tex <==
\section{Discussion}
\label{sec:discussion}

This study is not just a systemic review of the ML based approached to detect or diagnose AD in OCT and OCTA scans. We aimed to investigate the medical and technical background of the problem, existing technical proposals and application areas, and the requirements for future research. 

\todo{Boray Hocam buray biraz değiştirdim.}
We have extended the first research done by \cite{Bourkhime2022} by adding thesis and animal studies as well as unpublished archive journals. We came across five additional studies. Three of them were with animals on mice retinas. The only two studies that satisfied our initial intention were the recent work published by \cite{Wisely2022} and an older study published by \citep{Sandeep2019}. Even though there was an explosion of research using deep learning algorithms on OCT and OCTA data on various other diseases, lack of technical background or computational restrictions \citep{Yanagihara2020} could not be the root cause of this issue. We found excellent review articles and research studies on OCT images when we looked at the medical background. Various researchers tested the biomarkers, and they all agreed with the findings in sections \ref{OCT} and \ref{OCTA}. Therefore, lack of medical knowledge could be the root cause either. We observed that many use the same public datasets, such as \cite{Kermany2018, Pachade2021}. More are listed by \cite{Khan2021} in their dataset review study. Our results in this survey showed that the lack of publicly available OCT datasets was the significant root cause of the lack of AD screening from OCT and OCTA images. 

Our observation was also conclusive with a study by Yanagihara et al. \cite{Yanagihara2020}. Opthalmology has no global public dataset similar to Alzheimer’s Disease Neuroimaging Initiative (ADNI) \cite{ADNI}. Strict data privacy rules restricting the access. Publicly available medical data is priceless for academic research. UK Biobank offers its database for researchers for small fees. Many local data collection initiatives are going on, as seen in Table \ref{tbl:clinical_trials}.  AlzEye \cite{Wagner2022} is the largest dataset for ophthalmic images. It consists of longitudinal records of 353157 patients, which can even give more information about the progress of the disease. They recorded comprehensive demographic and ophthalmic data. (Fundus photograph, red-free photograph, fundus autofluorescence, pseudocolour photography (widefield) and optical coherence tomography).   

\cite{Yanagihara2020} also mentioned other data challenges of deep learning in OCT for retinal diseases, such as the lack of a standardized acquisition, image registration, and post-processing protocol. These challenges also limited the data set sizes and the capability of sharing/combining datasets. 

Finally, they discussed inconsistent metrics used in different studies that limit them. To overcome these issues and challenges Alzheimer’s Association in the United States  defined a ”minimum dataset” framework for SD-OCT retinal image acquisition and analysis. They support a collective initiative called the Atlas of Retinal Imaging in Alzheimer’s Study (ARIAS) \cite{Alber2020}. Although we also think these initiatives are valuable for future work, in our study, we saw those inconsistent metrics had not limited the number of other deep learning studies on OCT and OCTA images for other diseases. Instead these can be challenges and motivation for researchers to attack problems but not barriers to new research. Researchers need more publicly available datasets to build and test new models.

Deep Learning models are data hungry. Therefore most of the ML/DL studies \citep{Wisely2022, Tian2021, Lee2017,Thakoor2022} have used both eyes (left and right) to double the dataset size. We did not find any studies comparing the performance between training with single eyes vs both eyes. 

Currently, most of the research was done on 2D OCT slices. However, OCT devices generate 3D data. Increasing computational power and cloud services allow analyzing volumetric retinal images. Working with 3D OCT scans may also change the design of the problem and speed up the search results for the novel biomarkers. 

Despite their high performance, deep neural network architectures are black-box models. Trusting their predictions and the new biomarkers is essential in using them for decision-making in medicine. \cite{Ribeiro2016} raised the question "Why Should I Trust You?" and argued that people would trust a model more if they could understand the reasoning behind its predictions. \cite{Singh2021} evaluated 13 explainability deep learning methods for OCT scans. They assessed the Inception-v3 model that diagnoses three different diseases: choroidal neovascularization, diabetic macular oedema, and drusen. Their findings showed DTaylor outperforms the other methods in OCT retinal images. 

Alzheimer's Disease patients are aged people with more potential for multiple retinal diseases such as age-related macular degeneration \cite{Zhang2022}. There were various studies on deep learning-based multiple retinal disease detection on OCT/OCTA \cite{Ran2021}. Unfortunately, none of them included AD or MCI. In new data collection initiatives, multi-disease AD samples could also be included in the datasets to allow further studies on AD diagnosis with multi-retinal diseases. 

There were many retinal imaging modalities used for AD diagnosis. Vij et al. \cite{Vij2022} have systematically surveyed advances in these modalities. They  identified important discoveries and the pros/cons of using multi-modality images for AD detection. Wisely et al. \cite{Wisely2022} compared the performance of various modalities and  identified that patient data with OCT, with OCTA gives the best performance. OCT is a structural modality, while OCTA is a vascular one. Combining both of the features gave more information about the changes in the retina. 

Alzheimer's Disease is a prolonged progressing disease. Therefore detection of the disease in its early stages is vital. During our research, we observed that despite an increasing focus on early/mild cognitive impairment, there were no deep learning and/or machine learning studies on this topic. There were new data collection initiatives for MCI patients. Once these datasets are available, we expect to see more future studies on this topic.

==> tables_old.tex <==

%\begin{landscape}

\clearpage

\begin{table}
\centering
\caption{Development details of ML/DL models using OCT and OCTA data\\}

\resizebox{1\textwidth}{!}{% 

\begin{tabular}{ | m{1.6cm}| m{1.5cm}| m{2.4cm}| m{2cm}| m{4cm}| m{2.3cm}| m{3cm}| m{7cm}| } 

\hline
Author, Year, Reference  & Country & Source Data & Study Design & Main Variables & ML Algorithms & Validation method, feature detection (FS), data prepossessing (DP)  & Performance \\
\hline
\hline
Sayeed, 2022 & India & ACE College of Engineering, Trivandrum 695027, Kerala,& 24 triple transgenic mice more of AD , 2256 wild-type mice (HC) & Derived features from Fundus an OCT images & Decision Tree, Neural network, Random Forest, SVM & Validation method not specified, FS, DP & Decision Tree (96\% Acc., 94\% Sensitivity, 97\% Specifity)
Neural Network(74\% Acc., 98\% Sensitivity, 73\% Specifity)
Random Forest (98\% Acc., 65\% Sensitivity, 98\% Specifity)
SVM (99\% Acc., 98\% Sensitivity, 99\% Specifity) \\
\hline

Wisely, 2022 &	US & Duke University, NCT03233646 &	222 Eyes from 123 HC, 62 Eyes from 36 subjects with AD & Color maps of ganglion cell-inner flexiform layer (GC-IPL) thickness, superficial capillary plexus, OCTA images, and ultra-widefield (UWF) colour and fundus autoflourescence scanning lazer ophtalmoscopy images &	Convolutional Neural Networks (ResNet18) &	186 eyes for training and validating, 68 eyes for testing, FS, DP &	UWF colour AUC 0.450 (95\% CI 0.282, 0.592), OCTA SCP 0.582 (95\% CI 0.440, 0.724), UWF FAF 0.618 (95\% CI 0.462, 0.773), GC- IPL maps 0.809 (95\% CI 0.700, 0.919). A model incorporating all images, quantitative data and patient data (AUC 0.836 (CI 0.729, 0.943)) performed similarly to models only incorporating all images (AUC 0.829 (95\% CI 0.719, 0.939)). GC- IPL maps, quantitative data and patient data AUC 0.841 (95\% CI 0.739, 0.943) \\
\hline
Trindade, 2021 &	Spain	& the Coimbra Institute for Clinical and Biomedical Research (iCBR), Faculty of Medicine, University of Coimbra &	57 triple transgenic mice more of AD , 58 wild-type mice (HC) &	Fundus images + layer-aggregates Retinal Nerve Fibre Layer-Ganglion Cell Laye(RNFL-GCL), Inner Plexiform Layer(IPL), Inner Nuclear Layer(INL), Outer Plexiform Layer(OPL), and Total Retina(TR) &	Convolutional Neural Networks (Inception-v3) & five-fold cross validation &	6 CNNS trained separately resulted with accuracies between 79.0\% and 89.2
\\
\hline
Lemmens, 2020 &	Belgium & not available	& Cohort N=39 (10 AD, 7 amylod proven AD and 22 HC &	Amyloid accumulation and retinal nerve fiber layer thickness (RNFL) (retinal imaging hyperspectral snapshot camera + OCT) &	ML model not identified &	leave-one-out cross validation, FS, DP	& AUROC of 0.74
\\
\hline
Nunes, 2019	& Portugal	& Dementia and the movement Disorders Units of the Neurological Department of the Centro Hospitalare Universitaio de Coimbra &	Case-control, N=75 (20 AD, 28 PD, and 27 age-matched HC) &	Retinal texture+Retinal thickness (fundus images by OCT) Demographic data &	SVM	 & k-fold cross-validation, FS, DP	& "Sensitivity=88.7\%,
Specificity=84.9\%, Accuracy=82.2\%"\\
\hline
Zhou, 2006	& US &	N/A &	N/A	 & IRNF	& Artificial Neural Networks	& not available	& not available \\

\hline
\label{tbl:Results}%

\end{tabular}%

}
\end{table}



\clearpage

\begin{table*}
    \centering
    \caption{Alzheimer's Disease and OCT data collection initiatives based on ClinicalTrials.gov\\}
    \resizebox{1\textwidth}{!}{
    \begin{tabular}{|l|l|l|l|}
    \hline
        Study Title & Conditions & Interventions & Locations \\ \hline \hline
        1. Finding Retinal Biomarkers in Alzheimer's Disease & Alzheimer Disease & Other: Detailed ophthalmologic examination & Centre Mémoire de Ressources et \\ \hline
        ~ & ~ & ~ &  de Recherche Paris Nord, Paris, France \\ 
        2. Relationship Between Alzheimer Disease and  & Optical Coherence Tomography & Optical coherence tomography & CHU Amiens \\
        Diminution of the Three Macular Nervous  & Optical Coherence Tomography Ang. &  Optical coherence tomograpohy  & Amiens, France \\
    Retinal Layers & Retinal Thickening & angiography (OCTA) & ~ \\
        ~ & (and 5 more...) & ~ & ~ \\ \hline
        3. OCT Angiography and NRAI in Dementia & Alzheimer Disease & Optical Coherence Tomography Ang. & Oregon Health \& Science University \\ 
        ~ & Dementia &  (OCTA) Imaging & Portland, Oregon, United States \\ 
        ~ & Mild Cognitive Impairment & Noninvasive Retinal Amyloid Imaging (NRAI) & ~ \\ \hline
        4. The Role of Ophthalmologic Tests and EEG Imaging  & Mild Cognitive Impairment & Diagnostic Test: observational & Zhongshan Ophthalmic Center \\ 
        in Alzheimer's Disease & ~ & ~ & Guangzhou, Guangdong, China \\ \hline
        5. OCTA in Mild Cognitive Impairment and & Alzheimer Disease & Device: Retinal Imaging & Duke University Medical Center \\ 
         Alzheimer's Disease & Mild Cognitive Impairment & ~ & Durham, North Carolina, United States \\ 
        ~ & Retinal Vascular & ~ & ~ \\ 
        ~ & (and 4 more...) & ~ & ~ \\ \hline
        6. OCT-Angiography and Adaptive Optics in Patients  & Amnesia & Procedure: Ophthalmological exam & Hôpital Fondation A. de Rothschild \\ 
        With Memory Impairment & Alzheimer Disease & Procedure: Blood pressure measurement & Paris, France \\ 
        ~ & Lewy Body Disease & ~ & ~ \\
        ~ & Parkinsons Disease With Dementia & ~ & ~ \\ \hline
        7. Retinal Neuro-vascular Coupling in Patients  & Mild Cognitive Impairment & Device: DVA & Department of Clinical Pharmacology,  \\ 
        With Neurodegenerative Disease & Alzheimer Disease & Device: FDOCT & Medical University of Vienna \\
        ~ & Healthy & Device: Pattern ERG & Vienna, Austria \\
        ~ & ~ & Device: Optical Coherence Tomography & ~ \\ \hline
        8. BEAM: Brain-Eye Amyloid Memory Study & Alzheimer's Disease & Other: Pittsburgh Compound B [11C]-PIB & Sunnybrook Health Sciences Centre \\ 
        ~ & Mild Cognitive Impairment & ~ & Toronto, Ontario, Canada \\ 
        ~ & Vascular Cognitive Impairment & ~ & St. Michael's Hospital \\
        ~ & (and 2 more...) & ~ & Toronto, Ontario, Canada \\ 
        ~ & ~ & ~ & University Health Network \\
        ~ & ~ & ~ & Toronto, Ontario, Canada \\ 
        ~ & ~ & ~ & (and 2 more...) \\ \hline
        9. Atlas of Retinal Imaging in Alzheimer's Study & Alzheimer Disease & Other: Retinal Imaging & Morton Plant Hospital \\ 
        ~ & Mild Cognitive Impairment & Other: Pupillometry & Clearwater, Florida, United States \\ 
        ~ & Mild Dementia & Other: Contrast Sensitivity & St. Anthony's Hospital \\ 
        ~ & (and 2 more...) & (and 5 more...) & Saint Petersburg, Florida, United States \\ 
        ~ & ~ & ~ & University of Rhode Island \\ 
        ~ & ~ & ~ & Kingston, Rhode Island, United States \\
        ~ & ~ & ~ & Butler Hospital \\ 
        ~ & ~ & ~ & Providence, Rhode Island, United States \\ \hline
    \end{tabular}
  }
  \label{tbl:clinical_trials}

\end{table*}

%\end{landscape}
